Magnetogram-to-Magnetogram: Generative Forecasting of Solar Evolution

Investigating the solar magnetic field is crucial to understand the physical processes in the solar interior as well as their effects on the interplanetary environment. We introduce a novel method to predict the evolution of the solar line-of-sight (LoS) magnetogram using image-to-image translation with Denoising Diffusion Probabilistic Models (DDPMs). Our approach combines "computer science metrics" for image quality and "physics metrics" for physical accuracy to evaluate model performance. The results indicate that DDPMs are effective in maintaining the structural integrity, the dynamic range of solar magnetic fields, the magnetic flux and other physical features such as the size of the active regions, surpassing traditional persistence models, also in flaring situation. We aim to use deep learning not only for visualisation but as an integrative and interactive tool for telescopes, enhancing our understanding of unexpected physical events like solar flares. Future studies will aim to integrate more diverse solar data to refine the accuracy and applicability of our generative model.

==> library.tex <==
@article{Wiegelmann2014,
  author = {Wiegelmann, T. and Thalmann, J.K. and Solanki, S.K.},
  title = {The Magnetic Field in the Solar Atmosphere},
  journal = {Astronomy and Astrophysics Review},
  volume = {22},
  pages = {78},
  year = {2014},
  doi = {10.1007/s00159-014-0078-7},
  url = {https://doi.org/10.1007/s00159-014-0078-7}
}

@ARTICLE{sdo_telescope,
       author = {{Pesnell}, W. Dean and {Thompson}, B.~J. and {Chamberlin}, P.~C.},
        title = "{The Solar Dynamics Observatory (SDO)}",
      journal = {\solphys},
     keywords = {SDO, Solar cycle, Helioseismology, Coronal, Space weather},
         year = 2012,
        month = jan,
       volume = {275},
       number = {1-2},
        pages = {3-15},
          doi = {10.1007/s11207-011-9841-3},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SoPh..275....3P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hmi_instrument,
       author = {{Schou}, J. and {Scherrer}, P.~H. and {Bush}, R.~I. and {Wachter}, R. and {Couvidat}, S. and {Rabello-Soares}, M.~C. and {Bogart}, R.~S. and {Hoeksema}, J.~T. and {Liu}, Y. and {Duvall}, T.~L. and {Akin}, D.~J. and {Allard}, B.~A. and {Miles}, J.~W. and {Rairden}, R. and {Shine}, R.~A. and {Tarbell}, T.~D. and {Title}, A.~M. and {Wolfson}, C.~J. and {Elmore}, D.~F. and {Norton}, A.~A. and {Tomczyk}, S.},
        title = "{Design and Ground Calibration of the Helioseismic and Magnetic Imager (HMI) Instrument on the Solar Dynamics Observatory (SDO)}",
      journal = {\solphys},
     keywords = {Solar Dynamics Observatory, Helioseismology, observations, Instrumentation and data management, Magnetic fields, photosphere},
         year = 2012,
        month = jan,
       volume = {275},
       number = {1-2},
        pages = {229-259},
          doi = {10.1007/s11207-011-9842-2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SoPh..275..229S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{leka_a,
       author = {{Leka}, K.~D. and {Barnes}, G.},
        title = "{Photospheric Magnetic Field Properties of Flaring versus Flare-quiet Active Regions. I. Data, General Approach, and Sample Results}",
      journal = {\apj},
     keywords = {Sun: Activity, Sun: Flares, Sun: Photosphere, Techniques: Polarimetric},
         year = 2003,
        month = oct,
       volume = {595},
       number = {2},
        pages = {1277-1295},
          doi = {10.1086/377511},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...595.1277L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{leka_b,
       author = {{Leka}, K.~D. and {Barnes}, G.},
        title = "{Photospheric Magnetic Field Properties of Flaring versus Flare-quiet Active Regions. II. Discriminant Analysis}",
      journal = {\apj},
     keywords = {Methods: Statistical, Sun: Activity, Sun: Flares, Sun: Photosphere},
         year = 2003,
        month = oct,
       volume = {595},
       number = {2},
        pages = {1296-1306},
          doi = {10.1086/377512},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...595.1296L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{leka_c,
       author = {{Barnes}, G. and {Leka}, K.~D.},
        title = "{Photospheric Magnetic Field Properties of Flaring versus Flare-quiet Active Regions. III. Magnetic Charge Topology Models}",
      journal = {\apj},
     keywords = {Sun: Activity, Sun: Corona, Sun: Flares, Sun: Magnetic Fields, Sun: Photosphere},
         year = 2006,
        month = aug,
       volume = {646},
       number = {2},
        pages = {1303-1318},
          doi = {10.1086/504960},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...646.1303B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inbook{Pandey_2023,
   title={Explainable Deep Learning-Based Solar Flare Prediction with Post Hoc Attention for Operational Forecasting},
   ISBN={9783031452758},
   ISSN={1611-3349},
   url={http://dx.doi.org/10.1007/978-3-031-45275-8_38},
   DOI={10.1007/978-3-031-45275-8_38},
   booktitle={Lecture Notes in Computer Science},
   publisher={Springer Nature Switzerland},
   author={Pandey, Chetraj and Angryk, Rafal A. and Georgoulis, Manolis K. and Aydin, Berkay},
   year={2023},
   pages={567–581} }

@ARTICLE{Yi_et_al2023,
       author = {{Yi}, Kangwoo and {Moon}, Yong-Jae and {Jeong}, Hyun-Jin},
        title = "{Application of Deep Reinforcement Learning to Major Solar Flare Forecasting}",
      journal = {\apjs},
     keywords = {Solar flares, Neural networks, The Sun, 1496, 1933, 1693},
         year = 2023,
        month = apr,
       volume = {265},
       number = {2},
          eid = {34},
        pages = {34},
          doi = {10.3847/1538-4365/acb76d},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJS..265...34Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{COLLINS2021102383,
title = {Artificial intelligence in information systems research: A systematic literature review and research agenda},
journal = {International Journal of Information Management},
volume = {60},
pages = {102383},
year = {2021},
issn = {0268-4012},
doi = {https://doi.org/10.1016/j.ijinfomgt.2021.102383},
url = {https://www.sciencedirect.com/science/article/pii/S0268401221000761},
author = {Christopher Collins and Denis Dennehy and Kieran Conboy and Patrick Mikalef},
keywords = {Artificial intelligence, AI, Machine learning, Systematic literature review, Research agenda},
abstract = {AI has received increased attention from the information systems (IS) research community in recent years. There is, however, a growing concern that research on AI could experience a lack of cumulative building of knowledge, which has overshadowed IS research previously. This study addresses this concern, by conducting a systematic literature review of AI research in IS between 2005 and 2020. The search strategy resulted in 1877 studies, of which 98 were identified as primary studies and a synthesise of key themes that are pertinent to this study is presented. In doing so, this study makes important contributions, namely (i) an identification of the current reported business value and contributions of AI, (ii) research and practical implications on the use of AI and (iii) opportunities for future AI research in the form of a research agenda.}
}

@article{son2023three,

  title={Three-day Forecasting of Solar Wind Speed Using SDO/AIA Extreme-ultraviolet Images by a Deep-learning Model},

  author={Son, Jihyeon and Sung, Suk-Kyung and Moon, Yong-Jae and Lee, Harim and Jeong, Hyun-Jin},

  journal={The Astrophysical Journal Supplement Series},

  volume={267},

  number={2},

  pages={45},

  year={2023},

  publisher={IOP Publishing}

}

@article{jeong2020solar,

  title={Solar coronal magnetic field extrapolation from synchronic data with AI-generated farside},

  author={Jeong, Hyun-Jin and Moon, Yong-Jae and Park, Eunsu and Lee, Harim},

  journal={The Astrophysical Journal Letters},

  volume={903},

  number={2},

  pages={L25},

  year={2020},

  publisher={IOP Publishing}

}

@article{jeong2022improved,

title={Improved AI-generated Solar Farside Magnetograms by STEREO and SDO Data Sets and Their Release},

author={Jeong, Hyun-Jin and Moon, Yong-Jae and Park, Eunsu and Lee, Harim and Baek, Ji-Hye},

journal={The Astrophysical Journal Supplement Series},

volume={262},

number={2},

pages={50},

year={2022},

publisher={IOP Publishing}

}

@misc{kingma2022autoencoding,
      title={Auto-Encoding Variational Bayes}, 
      author={Diederik P Kingma and Max Welling},
      year={2022},
      eprint={1312.6114},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@misc{goodfellow2014generative,
      title={Generative Adversarial Networks}, 
      author={Ian J. Goodfellow and Jean Pouget-Abadie and Mehdi Mirza and Bing Xu and David Warde-Farley and Sherjil Ozair and Aaron Courville and Yoshua Bengio},
      year={2014},
      eprint={1406.2661},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@misc{ho2020denoising,
      title={Denoising Diffusion Probabilistic Models}, 
      author={Jonathan Ho and Ajay Jain and Pieter Abbeel},
      year={2020},
      eprint={2006.11239},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{rombach2022highresolution,
      title={High-Resolution Image Synthesis with Latent Diffusion Models}, 
      author={Robin Rombach and Andreas Blattmann and Dominik Lorenz and Patrick Esser and Björn Ommer},
      year={2022},
      eprint={2112.10752},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{saharia2022palette,
      title={Palette: Image-to-Image Diffusion Models}, 
      author={Chitwan Saharia and William Chan and Huiwen Chang and Chris A. Lee and Jonathan Ho and Tim Salimans and David J. Fleet and Mohammad Norouzi},
      year={2022},
      eprint={2111.05826},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{li2021srdiff,
      title={SRDiff: Single Image Super-Resolution with Diffusion Probabilistic Models}, 
      author={Haoying Li and Yifan Yang and Meng Chang and Huajun Feng and Zhihai Xu and Qi Li and Yueting Chen},
      year={2021},
      eprint={2104.14951},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{ramunno2024solar,
      title={Solar synthetic imaging: Introducing denoising diffusion probabilistic models on SDO/AIA data}, 
      author={Francesco P. Ramunno and S. Hackstein and V. Kinakh and M. Drozdova and G. Quetant and A. Csillaghy and S. Voloshynovskiy},
      year={2024},
      eprint={2404.02552},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@Article{s24041151,
AUTHOR = {Kinakh, Vitaliy and Belousov, Yury and Quétant, Guillaume and Drozdova, Mariia and Holotyak, Taras and Schaerer, Daniel and Voloshynovskiy, Slava},
TITLE = {Hubble Meets Webb: Image-to-Image Translation in Astronomy},
JOURNAL = {Sensors},
VOLUME = {24},
YEAR = {2024},
NUMBER = {4},
ARTICLE-NUMBER = {1151},
URL = {https://www.mdpi.com/1424-8220/24/4/1151},
PubMedID = {38400307},
ISSN = {1424-8220},
ABSTRACT = {This work explores the generation of James Webb Space Telescope (JWSP) imagery via image-to-image translation from the available Hubble Space Telescope (HST) data. Comparative analysis encompasses the Pix2Pix, CycleGAN, TURBO, and DDPM-based Palette methodologies, assessing the criticality of image registration in astronomy. While the focus of this study is not on the scientific evaluation of model fairness, we note that the techniques employed may bear some limitations and the translated images could include elements that are not present in actual astronomical phenomena. To mitigate this, uncertainty estimation is integrated into our methodology, enhancing the translation’s integrity and assisting astronomers in distinguishing between reliable predictions and those of questionable certainty. The evaluation was performed using metrics including MSE, SSIM, PSNR, LPIPS, and FID. The paper introduces a novel approach to quantifying uncertainty within image translation, leveraging the stochastic nature of DDPMs. This innovation not only bolsters our confidence in the translated images but also provides a valuable tool for future astronomical experiment planning. By offering predictive insights when JWST data are unavailable, our approach allows for informed preparatory strategies for making observations with the upcoming JWST, potentially optimizing its precious observational resources. To the best of our knowledge, this work is the first attempt to apply image-to-image translation for astronomical sensor-to-sensor translation.},
DOI = {10.3390/s24041151}
}

@article{mariia_drozdova,
	author = {{Drozdova, M.} and {Kinakh, V.} and {Bait, O.} and {Taran, O.} and {Lastufka, E.} and {Dessauges-Zavadsky, M.} and {Holotyak, T.} and {Schaerer, D.} and {Voloshynovskiy, S.}},
	title = {Radio-astronomical image reconstruction with a conditional denoising diffusion model⋆},
	DOI= "10.1051/0004-6361/202347948",
	url= "https://doi.org/10.1051/0004-6361/202347948",
	journal = {A&A},
	year = 2024,
	volume = 683,
	pages = "A105",
}

@article{jarolim_2024,
author = {Jarolim, Robert and Tremblay, Benoit and Munoz-Jaramillo, Andres and Bintsi, Kyriaki-Margarita and Jungbluth, Anna and Santos, Miraflor and Vourlidas, Angelos and Mason, James and Sundaresan, Sairam and Downs, Cooper and Caplan, Ronald},
year = {2024},
month = {01},
pages = {L31},
title = {SuNeRF: 3D Reconstruction of the Solar EUV Corona Using Neural Radiance Fields},
volume = {961},
journal = {The Astrophysical Journal Letters},
doi = {10.3847/2041-8213/ad12d2}
}

@misc{dhariwal2021diffusion,
      title={Diffusion Models Beat GANs on Image Synthesis}, 
      author={Prafulla Dhariwal and Alex Nichol},
      year={2021},
      eprint={2105.05233},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{Plutino_2023,
   title={A new catalogue of solar flare events from soft X-ray GOES signal in the period 1986–2020},
   volume={71},
   ISSN={0273-1177},
   url={http://dx.doi.org/10.1016/j.asr.2022.11.020},
   DOI={10.1016/j.asr.2022.11.020},
   number={4},
   journal={Advances in Space Research},
   publisher={Elsevier BV},
   author={Plutino, Nicola and Berrilli, Francesco and Del Moro, Dario and Giovannelli, Luca},
   year={2023},
   month=feb, pages={2048–2058} }

@misc{zhang2018unreasonable,
      title={The Unreasonable Effectiveness of Deep Features as a Perceptual Metric}, 
      author={Richard Zhang and Phillip Isola and Alexei A. Efros and Eli Shechtman and Oliver Wang},
      year={2018},
      eprint={1801.03924},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@ARTICLE{ssim,
  author={Zhou Wang and Bovik, A.C. and Sheikh, H.R. and Simoncelli, E.P.},
  journal={IEEE Transactions on Image Processing}, 
  title={Image quality assessment: from error visibility to structural similarity}, 
  year={2004},
  volume={13},
  number={4},
  pages={600-612},
  keywords={Image quality;Humans;Transform coding;Visual system;Visual perception;Data mining;Layout;Quality assessment;Degradation;Indexes},
  doi={10.1109/TIP.2003.819861}}

@misc{delbracio2024inversion,
      title={Inversion by Direct Iteration: An Alternative to Denoising Diffusion for Image Restoration}, 
      author={Mauricio Delbracio and Peyman Milanfar},
      year={2024},
      eprint={2303.11435},
      archivePrefix={arXiv},
      primaryClass={eess.IV}
}

@ARTICLE{sunpy,
  doi = {10.3847/1538-4357/ab4f7a},
  url = {https://iopscience.iop.org/article/10.3847/1538-4357/ab4f7a},
  author = {{The SunPy Community} and Barnes, Will T. and Bobra, Monica G. and Christe, Steven D. and Freij, Nabil and Hayes, Laura A. and Ireland, Jack and Mumford, Stuart and Perez-Suarez, David and Ryan, Daniel F. and Shih, Albert Y. and Chanda, Prateek and Glogowski, Kolja and Hewett, Russell and Hughitt, V. Keith and Hill, Andrew and Hiware, Kaustubh and Inglis, Andrew and Kirk, Michael S. F. and Konge, Sudarshan and Mason, James Paul and Maloney, Shane Anthony and Murray, Sophie A. and Panda, Asish and Park, Jongyeob and Pereira, Tiago M. D. and Reardon, Kevin and Savage, Sabrina and Sipőcz, Brigitta M. and Stansby, David and Jain, Yash and Taylor, Garrison and Yadav, Tannmay and Rajul and Dang, Trung Kien},
  title = {The SunPy Project: Open Source Development and Status of the Version 1.0 Core Package},
  journal = {The Astrophysical Journal},
  volume = {890},
  issue = {1},
  pages = {68-},
  publisher = {American Astronomical Society},
  year = {2020}
}

@article{Sadykov_2017,
   title={Relationships between Characteristics of the Line-of-sight Magnetic Field and Solar Flare Forecasts},
   volume={849},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/1538-4357/aa9119},
   DOI={10.3847/1538-4357/aa9119},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Sadykov, Viacheslav M. and Kosovichev, Alexander G.},
   year={2017},
   month=nov, pages={148} }

@ARTICLE{wang_2020,
       author = {{Wang}, Jingjing and {Zhang}, Yuhang and {Hess Webber}, Shea A. and {Liu}, Siqing and {Meng}, Xuejie and {Wang}, Tieyan},
        title = "{Solar Flare Predictive Features Derived from Polarity Inversion Line Masks in Active Regions Using an Unsupervised Machine Learning Algorithm}",
      journal = {\apj},
     keywords = {Solar flares, Space weather, Classification, Solar active regions, 1496, 2037, 1907, 1974},
         year = 2020,
        month = apr,
       volume = {892},
       number = {2},
          eid = {140},
        pages = {140},
          doi = {10.3847/1538-4357/ab7b6c},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...892..140W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{jaccard,
author = {Jaccard, Paul},
year = {1901},
month = {01},
pages = {547-579},
title = {Etude de la distribution florale dans une portion des Alpes et du Jura},
volume = {37},
journal = {Bulletin de la Societe Vaudoise des Sciences Naturelles},
doi = {10.5169/seals-266450}
}

@inproceedings{pil,
author = {Cai, Xumin and Aydin, Berkay and Ji, Anli and Georgoulis, Manolis and Angryk, Rafal},
year = {2020},
month = {12},
pages = {4175-4183},
title = {A Framework for Detecting Polarity Inversion Lines from Longitudinal Magnetograms},
doi = {10.1109/BigData50022.2020.9377808}
}

@misc{menon2020pulse,
      title={PULSE: Self-Supervised Photo Upsampling via Latent Space Exploration of Generative Models}, 
      author={Sachit Menon and Alexandru Damian and Shijia Hu and Nikhil Ravi and Cynthia Rudin},
      year={2020},
      eprint={2003.03808},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{NIPS2012_c399862d,
 author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {F. Pereira and C.J. Burges and L. Bottou and K.Q. Weinberger},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {ImageNet Classification with Deep Convolutional Neural Networks},
 url = {https://proceedings.neurips.cc/paper_files/paper/2012/file/c399862d3b9d6b76c8436e924a68c45b-Paper.pdf},
 volume = {25},
 year = {2012}
}

@article{helioviewer,
author = {Ireland, Jonathan and Hughitt, Vincent and Müller, D. and Dimitoglou, George and Schmiedel, P. and Fleck, Bernhard},
year = {2009},
month = {04},
pages = {},
title = {The Helioviewer Project: Discovery For Everyone Everywhere},
volume = {40}
}

@ARTICLE{kleint_lucia,
       author = {{Kleint}, Lucia},
        title = "{First Detection of Chromospheric Magnetic Field Changes during an X1-Flare}",
      journal = {\apj},
     keywords = {Sun: chromosphere, Sun: flares, Sun: magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.3847/1538-4357/834/1/26},
archivePrefix = {arXiv},
       eprint = {1608.02552},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834...26K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Sun_2022,
   title={Predicting Solar Flares Using CNN and LSTM on Two Solar Cycles of Active Region Data},
   volume={931},
   ISSN={1538-4357},
   url={http://dx.doi.org/10.3847/1538-4357/ac64a6},
   DOI={10.3847/1538-4357/ac64a6},
   number={2},
   journal={The Astrophysical Journal},
   publisher={American Astronomical Society},
   author={Sun, Zeyu and Bobra, Monica G. and Wang, Xiantong and Wang, Yu and Sun, Hu and Gombosi, Tamas and Chen, Yang and Hero, Alfred},
   year={2022},
   month=jun, pages={163} }

@inbook{Pandey_2023,
   title={Explainable Deep Learning-Based Solar Flare Prediction with Post Hoc Attention for Operational Forecasting},
   ISBN={9783031452758},
   ISSN={1611-3349},
   url={http://dx.doi.org/10.1007/978-3-031-45275-8_38},
   DOI={10.1007/978-3-031-45275-8_38},
   booktitle={Lecture Notes in Computer Science},
   publisher={Springer Nature Switzerland},
   author={Pandey, Chetraj and Angryk, Rafal A. and Georgoulis, Manolis K. and Aydin, Berkay},
   year={2023},
   pages={567–581} }

@ARTICLE{panos,
       author = {{Panos}, Brandon and {Kleint}, Lucia and {Zbinden}, Jonas},
        title = "{Identifying preflare spectral features using explainable artificial intelligence}",
      journal = {\aap},
     keywords = {Sun: flares, techniques: spectroscopic, Sun: activity, Sun: chromosphere, methods: data analysis, methods: statistical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = mar,
       volume = {671},
          eid = {A73},
        pages = {A73},
          doi = {10.1051/0004-6361/202244835},
archivePrefix = {arXiv},
       eprint = {2301.01560},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...671A..73P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{GEORGOULIS2024,
title = {Prediction of solar energetic events impacting space weather conditions},
journal = {Advances in Space Research},
year = {2024},
issn = {0273-1177},
doi = {https://doi.org/10.1016/j.asr.2024.02.030},
url = {https://www.sciencedirect.com/science/article/pii/S027311772400173X},
author = {Manolis K. Georgoulis and Stephanie L. Yardley and Jordan A. Guerra and Sophie A. Murray and Azim Ahmadzadeh and Anastasios Anastasiadis and Rafal Angryk and Berkay Aydin and Dipankar Banerjee and Graham Barnes and Alessandro Bemporad and Federico Benvenuto and D. Shaun Bloomfield and Monica Bobra and Cristina Campi and Enrico Camporeale and Craig E. DeForest and A. Gordon Emslie and David Falconer and Li Feng and Weiqun Gan and Lucie M. Green and Sabrina Guastavino and Mike Hapgood and Dustin Kempton and Irina Kitiashvili and Ioannis Kontogiannis and Marianna B. Korsos and K.D. Leka and Paolo Massa and Anna Maria Massone and Dibyendu Nandy and Alexander Nindos and Athanasios Papaioannou and Sung-Hong Park and Spiros Patsourakos and Michele Piana and Nour E. Rawafi and Viacheslav M. Sadykov and Shin Toriumi and Angelos Vourlidas and Haimin Wang and Jason T. {L. Wang} and Kathryn Whitman and Yihua Yan and Andrei N. Zhukov},
keywords = {International space weather action teams, Forecasting, Solar flares and eruptions, Methods – statistical, Methods – machine learning, Future missions},
abstract = {Aiming to assess the progress and current challenges on the formidable problem of the prediction of solar energetic events since the COSPAR/ International Living With a Star (ILWS) Roadmap paper of Schrijver et al. (2015), we attempt an overview of the current status of global research efforts. By solar energetic events we refer to flares, coronal mass ejections (CMEs), and solar energetic particle (SEP) events. The emphasis, therefore, is on the prediction methods of solar flares and eruptions, as well as their associated SEP manifestations. This work complements the COSPAR International Space Weather Action Teams (ISWAT) review paper on the understanding of solar eruptions by Linton et al. (2023) (hereafter, ISWAT review papers are conventionally referred to as ’Cluster’ papers, given the ISWAT structure). Understanding solar flares and eruptions as instabilities occurring above the nominal background of solar activity is a core solar physics problem. We show that effectively predicting them stands on two pillars: physics and statistics. With statistical methods appearing at an increasing pace over the last 40 years, the last two decades have brought the critical realization that data science needs to be involved, as well, as volumes of diverse ground- and space-based data give rise to a Big Data landscape that cannot be handled, let alone processed, with conventional statistics. Dimensionality reduction in immense parameter spaces with the dual aim of both interpreting and forecasting solar energetic events has brought artificial intelligence (AI) methodologies, in variants of machine and deep learning, developed particularly for tackling Big Data problems. With interdisciplinarity firmly present, we outline an envisioned framework on which statistical and AI methodologies should be verified in terms of performance and validated against each other. We emphasize that a homogenized and streamlined method validation is another open challenge. The performance of the plethora of methods is typically far from perfect, with physical reasons to blame, besides practical shortcomings: imperfect data, data gaps and a lack of multiple, and meaningful, vantage points of solar observations. We briefly discuss these issues, too, that shape our desired short- and long-term objectives for an efficient future predictive capability. A central aim of this article is to trigger meaningful, targeted discussions that will compel the community to adopt standards for performance verification and validation, which could be maintained and enriched by institutions such as NASA’s Community Coordinated Modeling Center (CCMC) and the community-driven COSPAR/ISWAT initiative.}
}

@article{opencv_library,
    author = {Bradski, G.},
    citeulike-article-id = {2236121},
    journal = {Dr. Dobb's Journal of Software Tools},
    keywords = {bibtex-import},
    posted-at = {2008-01-15 19:21:54},
    priority = {4},
    title = {{The OpenCV Library}},
    year = {2000}
}
